Characterizing consensus in the Heard-Of model

The Heard-Of model is a simple and relatively expressive model of distributed computation. Because of this, it has gained a considerable attention of the verification community. We give a characterization of all algorithms solving consensus in a fragment of this model. The fragment is big enough to cover many prominent consensus algorithms. The characterization is purely syntactic: it is expressed in terms of some conditions on the text of the algorithm. One of the recent methods of verification of distributed algorithms is to abstract an algorithm to the Heard-Of model and then to verify the abstract algorithm using semi-automatic procedures. Our results allow, in some cases, to avoid the second step in this methodology.

==> app-examples.tex <==
\section{Other examples of algorithms covered by our characterizations}
\label{sec:app-examples}

In this section present some other known algorithms that fit into our fragment
of the Heard-Of model. 
We also show their variants that are correct by our characterization.
Finally, we a show new algorithm written in the core language, i.e., without
time-stamps and coordinators.



\begin{algorithm}[H]\label{alg:one-third-more-parameters}
	%\SetAlgoLined
		\Send{$(\inp)$}{
		\lIf{$\uni(\ho) \land |\ho| > \thru^1 \cdot |\Pi|$}{$x_1:=\inp:=\smor(\ho)$}
		\lIf{$\mult(\ho) \land |\ho| > \thrm^1 \cdot |\Pi|$}{$x_1:=\inp:=\smor(\ho)$}
	}
	\Send{$x_1$}{
		\lIf{$\uni(\ho) \land |\ho| > \thru^2 \cdot |\Pi|$}{$\dec:=\smor(\ho)$}
	}
	\BlankLine
	\Cp{$\lF(\p^1 \land \lF\p^2)$}
	%\Where{$\p^1 := (\f_{=}\land\f_{\thr_1},\true)$\quad and\quad $\p^2 := (\f_{\thr_1},\f_{\thr_2})$}
	\caption{Parametrized OneThird algorithm~\cite{charron-heard-distributed09}, $\thru^1$, $\thrm^1, \thru^2$ are constants from $(0,1)$}
\end{algorithm}

\igw{added analysis of the characterization for the core language.} 
Let us list all the constraints on the constants that would make this algorithm
solve consensus. 
Observe, that if we want an algorithm with 2 rounds, by structural constraints
from Definition~\ref{def:structure}, there must be $\mult$ instruction in the
first round and there cannot be $\mult$ instruction in the second round.
The operation in the $\mult$ instruction must be $\smor$.
Both rounds need to have $\uni$ instruction.

The structural constraints from Definition~\ref{def:structure} say
\begin{equation*}
	\thrm^1/2\geq 1-\thru^2 \quad\text{and}\quad \thru^1\geq 1-\thru^2
\end{equation*}
Recall that the formula for border threshold is
\begin{equation*}
	\bthr= \max(1-\thruo,1-\thrmok/2)	
\end{equation*}

We will consider only the case when the global predicate is $(\true,\true)$ so
there are no constraints coming from the proviso. 
Let us see what can be $\p^1$ and $\p^2$ so that we have a unifier and a
decider.

Decider is a simpler one. 
We need to have $\p^2:=(\f_{\thru^1},\f_{\thru^2})$ or some bigger thresholds.

For a unifier we need $\p^1:=(\f_{=}\land\f_{\th},\true)$, but we may have a
choice for $\th$ with respect to the constants $\thru^1, \thrm^1, \thru^2$. 
\begin{itemize}
	\item Suppose $\thru^1\leq \thrm^1$. Then the constraints on unifier reduce to $\th\geq\thrm^1$.
	\item Suppose $\thru^1>\thrm^1$ and all the constrains for the algorithm to
	solve consensus are satisfied. Then we can
	decrease $\thru^1$ to $\thrm^1$, and they will be still satisfied. Actually,
	one can show that one can decrease $\thru^1$ to $\thrm^1/2$. 
\end{itemize}

To sum up the constraints are $\th\geq\thrm^1$, $\thru^1=\thrm^1/2\geq 1
-\thru^2$. 
If we want to keep the constants as small as possible we take $\th=\thrm^1$.
We get the best constraints as a function of $\thrm^1$:
\begin{equation*}
	\p^1=(\f_{=}\land\f_{\thrm^1},\true)\qquad \p^2=(\thrm^1/2,1-\thrm^1)
\end{equation*}




\begin{algorithm}[H]\label{alg:new-timestamp}
	%\SetAlgoLined
		\Send{$(\inp,ts)$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_1:=\maxts(\ho)$}
		\lIf{$\mult(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_1:=\maxts(\ho)$}
	}
	\Send{$x_1$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_2:=\inp:=\smor(\ho)$}
	}
	\Send{$x_2$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$\dec:=\smor(\ho)$}
	}
	\BlankLine
	\Cp{$\lF(\p^1)$ where $\p^1 := (\f_=\land\f_{1/2},\ \f_{1/2},\ \f_{1/2})$}
	\caption{A timestamp algorithm from~\cite{Mar:17}}
\end{algorithm}
This algorithm is correct by Theorem~\ref{thm:ts}. 
The theorem also says that the communication predicate can be weakened to
$\lF(\p^1\land\lF\p^2)$ where $\p^1=(\f_=\land\f_{1/2},\ \f_{1/2},\ \true)$
and $\p^2=(\f_{1/2},\ \f_{1/2},\ \f_{1/2})$.
\medskip


If we do not want to have $\f_=$ requirement on the first line where we check
timestamps, we can consider the following modification of the above.
%\bala{Modified this, because the previous algorithm was not correct.}

\begin{algorithm}[H]\label{alg:mod-new-timestamp} 
	%\SetAlgoLined
		\Send{$(\inp,ts)$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_1:=\maxts(\ho)$}
		\lIf{$\mult(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_1:=\maxts(\ho)$}
	}
	\Send{$x_1$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_2:=\smor(\ho)$}
		\lIf{$\mult(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_2:=\smor(\ho)$}
	}
	\Send{$x_2$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_3:=\inp:=\smor(\ho)$}
	}
	\Send{$x_3$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$\dec:=\smor(\ho)$}
	}
	\BlankLine
	\Cp{$\lF(\p^1\land\lF\p^2)$}
	\Where{$\p^1=(\f_{1/2},\ \f_=\land\f_{1/2}, \ \f_{1/2}, \ \true)$
	and $\p^2=(\f_{1/2},\ \f_{1/2},\ \f_{1/2}, \ \f_{1/2})$}
	\caption{A modification of a timestamp algorithm from~\cite{Mar:17}}
\end{algorithm}
Note that by Theorem~\ref{thm:ts}, when we move the equalizer to the
second round, there necessarily has to be a $\mult$ instruction in the
second round.

\begin{comment}
If we could set $\inp$ in the first line, we can have even shorter
algorithm

\begin{algorithm}[H]\label{alg:short-timestamp}
	%\SetAlgoLined
		\Send{$(\inp,ts)$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$\inp:=x_1:=\maxts(\ho)$}
		\lIf{$\mult(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$\inp:=x_1:=\maxts(\ho)$}
	}
	\Send{$x_2$ $\every$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$\dec:=\smor(\ho)$}
	}
	\BlankLine
	\Cp{$\lF(\p^1\land\lF\p^2)$}
	\Where{$\p^1=(\f_=\land\f_{1/2},\ \true)$
	and $\p^2=(\f_{1/2},\  \f_{1/2})$}
	\caption{A short timestamp algorithm}
\end{algorithm}
\end{comment}
%\balain[Removed the previous algorithm as it was not correct by Lemma~\ref{lem:ts-min}]
\medskip

The next example is a three round version of Paxos algorithm. 

\begin{algorithm}[H]\label{alg:paxos-three}
	%\SetAlgoLined
		\Send{$(\inp,ts)$ $\lr$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_1:=\maxts(\ho)$}
		\lIf{$\mult(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$x_1:=\maxts(\ho)$}
	}
	\Send{$x_1$ $\ls$}{
		\lIf{$\uni(\ho)$}{$x_2:=\inp:=\smor(\ho)$}
	}
	\Send{$x_2$ $\every$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/2 \cdot |\Pi|$}{$\dec:=\smor(\ho)$}
	}
	\BlankLine
	\Cp{$\lF(\p^1)$ where $\p^1 := (\f_{1/2},\ \f_{\ls},\ \f_{1/2})$}
	\caption{Three round Paxos algorithm}
\end{algorithm}
The algorithm is correct by Theorem~\ref{thm:ts-coordinators}. 
Once again it is possible to change constants in the first round to $1/3$ and in
the last round to $2/3$ (both in the algorithm and in the communication predicate).
\bigskip

One \igw{New algorithm} can ask if it is possible to have an algorithm with coordinators without
timestamps.
Here is a possibility that resembles three round Paxos:

\begin{algorithm}[H]\label{alg:paxos-coordinators}
	%\SetAlgoLined
		\Send{$(\inp)$ $\lr$}{
		\lIf{$\uni(\ho) \land |\ho| > 2/3 \cdot |\Pi|$}{$x_1:=\smor(\ho)$}
		\lIf{$\mult(\ho) \land |\ho| > 2/3 \cdot |\Pi|$}{$x_1:=\smor(\ho)$}
	}
	\Send{$x_1$ $\ls$}{
		\lIf{$\uni(\ho)$}{$x_2:=\inp:=\smor(\ho)$}
	}
	\Send{$x_2$ $\every$}{
		\lIf{$\uni(\ho) \land |\ho| > 2/3 \cdot |\Pi|$}{$\dec:=\smor(\ho)$}
	}
	\BlankLine
	\Cp{$\lF(\p)$\quad where $\p := (\f_{2/3},\f_{\ls},\f_{2/3})$}
			\caption{Three round coordinator algorithm}
\end{algorithm}
The algorithm solves consensus by Theorem~\ref{thm:coordinators}. 
The constants are bigger than in Paxos because we do not have timestamps: 
the constraints on constants come from
Definition~\ref{def:structure}, and not from Definition~\ref{def:ts-structure}. 
We can parametrize this algorithm in the same way as we did for
Algorithm~\ref{alg:one-third}. \\


Chandra-Toueg algorithm in the Heard-Of model is actually syntactically the same
as four round Paxos~\cite{Mar:17}. 
The communication predicate is even stronger so it clearly satisfies our constraints.\\


The notion of a weak unifier from Theorem~\ref{thm:core} seems to be a new. 
Here is an algorithm that has  a weak unifier, but does not have a strong
unifier. 
The algorithm is probably not the most efficient one but it is not the same as
the others. 

\begin{algorithm}[H]\label{alg:weak-unifier}
	\Send{$\inp$}{
		\lIf{$\uni(\ho) \land |\ho| > 9/10 \cdot |\Pi|$}{$x_1:=\smor(\ho)$}
		\lIf{$\mult(\ho) \land |\ho| > 4/5 \cdot |\Pi|$}{$x_1:=\smor(\ho)$}
	}
	\Send{$x_1$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/100 \cdot |\Pi|$}{$x_2:=\inp:=\min(\ho)$}
		\lIf{$\mult(\ho) \land |\ho| > 1/100 \cdot |\Pi|$}{$x_2:=\inp:=\min(\ho)$}
	}
	\Send{$x_2$}{
		\lIf{$\uni(\ho) \land |\ho| > 3/5 \cdot |\Pi|$}{$x_3:=\min(\ho)$}
	}
	\Send{$x_3$}{
		\lIf{$\uni(\ho) \land |\ho| > 1/100 \cdot |\Pi|$}{$\dec:=\smor(\ho)$}
	}
	\BlankLine
	\Cp{$\lF(\p^1\land\lF\p^2)$}
	\Where{$\p^1=(\f_=\land\f_{4/5},\ \f_{1/100},\ \true,\ \true)$ and
		$\p^2 = (\f_{9/10},\ \f_{1/100}, \ \f_{3/5},\ \f_{1/100})$}
	\caption{An algorithm with a weak unifier}
\end{algorithm}
Clearly $\p^1$ is a weak-unifier and $\p^2$ is both a finalizer 
and a decider. 
\bigskip

% Here is another example that follows Theorem~\ref{thm:core}. 
% Observe that the algorithm solves consensus in a single phase if
% all the processes have the same initial value.

% \begin{algorithm}[H]\label{alg:fast-solo}
% 	\Send{$\inp$}{
% 		\lIf{$\uni(\ho) \land |\ho| > 1/3 \cdot |\Pi|$}{$x_1:=\smor(\ho)$}
% 		\lIf{$\mult(\ho) \land |\ho| > 2/3 \cdot |\Pi|$}{$x_1:=\smor(\ho)$}
% 	}
% 	\Send{$x_1$}{
% 		\lIf{$\uni(\ho) \land |\ho| > 1/100 \cdot |\Pi|$}{$x_2:=\inp:=\min(\ho)$}
% 		\lIf{$\mult(\ho) \land |\ho| > 1/100 \cdot |\Pi|$}{$x_2:=\inp:=\min(\ho)$}
% 	}
% 	\Send{$x_2$}{
% 		\lIf{$\uni(\ho) \land |\ho| > 2/3 \cdot |\Pi|$}{$x_3:=\min(\ho)$}
% 	}
% 	\Send{$x_3$}{
% 		\lIf{$\uni(\ho) \land |\ho| > 1/100 \cdot |\Pi|$}{$\dec:=\smor(\ho)$}
% 	}
% 	\BlankLine
% 	\Cp{$\lG\p \land \lF(\p^1\land\lF\p^2)$}
% 	\Where{$\p = (\f_{1/3},\f_{1/100},\f_{2/3},\f_{1/100})$,
% 		$\p^1=(\f_=\land\f_{2/3},\ \f_{1/100},\ \f_{2/3},\ \f_{1/100})$}
% 	\caption{An one-step consensus algorithm}
% \end{algorithm}
% \igwin{Why do we need $\p^2$? Already $\p^1$ is strong equalizer and decider?}
% \balain[You are completely right. I had overlooked it and now I have 
% 	corrected it.]
% 	\igwin{Your correction changes nothing because of the global predicate.}
% \balain[Modified to take into account the global predicate.]




% \subsection{OneThird algorithm (Variant) \cite{HO}}

% \emph{Comm. predicate: } $\lF(\p^1 \land \lF(\p^2))$ where
% \begin{itemize}
% 	\item $\p^1 := (\f_{2/3,=},\true)$
% 	\item $\p^2 := (\f_{2/3},\f_{2/3})$
% \end{itemize}
% \begin{align*}
% \send(\inp) \\
% &\iif\ \uni(\ho) \land |\ho| > 2/3 \cdot |\Pi| \ \tthen\ x_1:=\inp:=\smor(\ho)\\
% &\iif\ \mult(\ho) \land |\ho| > 2/3 \cdot |\Pi| \ \tthen\ x_1:=\inp:=\smor(\ho)
% \end{align*}
% \begin{align*}
% \send(x_1) \\
% &\iif\ \uni(\ho) \land |\ho| > 2/3 \cdot |\Pi| \ \tthen\ \dec:=\smor(\ho)
% \end{align*}

% The algorithm satisfies our assumptions and is correct by theorem \ref{thm:core}.

% \subsection{$\mathcal{A}_{T,E}$ algorithm (variant)}

% In the paper introducing Heard-of model~\cite{charron-heard-distributed09},
% Charron-Bost and Schiper ask if there is a way to use smaller constants than 2/3.
% In our terms they ask if there is an algorithm in the core language with trivial
% global predicate that uses the constants smaller than $2/3$ employed by OneThird
% algorithm. 
% To answer this question we can take the OneThird algorithm and  parametrize the
% thresholds for the two  rounds: we use $T$ and $E$ below.
% Our characterization (Theorem~\ref{thm:core}) gives us all possible pairs of $(T,E)$ for
% which the resulting algorithm solves consensus: they should satisfy $T \ge
% 2(1-E)$\igw{and maybe something more?}.


% \emph{Comm. predicate: } $\lF(\p^1 \land \lF(\p^2))$ where
% \begin{itemize}
% 	\item $\p^1 := (\f_{T,=},\true)$
% 	\item $\p^2 := (\f_{T},\f_{E})$
% \end{itemize}
% \begin{align*}
% \send(\inp) \\
% &\iif\ \uni(\ho) \land |\ho| > T \cdot |\Pi| \ \tthen\ x_1:=\inp:=\smor(\ho)\\
% &\iif\ \mult(\ho) \land |\ho| > T \cdot |\Pi| \ \tthen\ x_1:=\inp:=\smor(\ho)
% \end{align*}
% \begin{align*}
% \send(x_1) \\
% &\iif\ \uni(\ho) \land |\ho| > E \cdot |\Pi| \ \tthen\ \dec:=\smor(\ho)
% \end{align*}

% Here $T$ and $E$ are such that .
% The algorithm satisfies our assumptions and is correct by theorem \ref{thm:core}.





% \subsection{New timestamp algorithm \cite{Thesis}}



% \emph{Comm. predicate: } $\lF \p$ where 
% \begin{align*}
% \send(\inp,\ts) \\
% &\iif\ \uni(\ho) \land |\ho| > 1/2 \cdot |\Pi| \ \tthen\ x_1:=\maxts(\ho)\\
% &\iif\ \mult(\ho) \land |\ho| > 1/2 \cdot |\Pi| \ \tthen\ x_1:=\maxts(\ho)
% \end{align*}
% \begin{align*}
% \send(x_1) \\
% &\iif\ \uni(\ho) \land |\ho| > 1/2 \cdot |\Pi| \ \tthen\ x_2:=\inp:=\smor(\ho)
% \end{align*}
% \begin{align*}
% \send(x_2) \\
% &\iif\ \uni(\ho) \land |\ho| > 1/2 \cdot |\Pi| \ \tthen\ \dec:=\smor(\ho)
% \end{align*}

% The algorithm satisfies our assumptions and is correct by theorem
% \ref{thm:ts}.


% \subsection{Paxos}






